The Quark and Gluon Structure of the Proton

In this article we present a review of the structure of the proton and the current status of our knowledge of the parton distribution functions (PDFs). The lepton-nucleon scattering experiments which provide the main constraints in PDF extractions are introduced and their measurements are discussed. Particular emphasis is given to the HERA data which cover a wide kinematic region. Hadron-hadron scattering measurements which provide supplementary information are also discussed. The methods used by various groups to extract the PDFs in QCD analyses of hard scattering data are presented and their results are compared. The use of existing measurements allows predictions for cross sections at the LHC to be made. A comparison of these predictions for selected processes is given. First measurements from the LHC experiments are compared to predictions and some initial studies of the impact of this new data on the PDFs are presented.

==> Makefile <==
F_FLAGS = -g
C_FLAGS = -w -O0 -D_GNU_SOURCE -Df2cFortran -fpic 
COMP    = -fno-globals -fno-automatic -finit-local-zero 
F77LIB =gfortran
F77COMP=gfortran



ReviewPaper: 
	latex ReviewPaper
	latex ReviewPaper
	latex ReviewPaper
	dvips ReviewPaper
	ps2pdf ReviewPaper.ps ReviewPaper.pdf
#	open ReviewPaper.pdf

ReviewPaperPDF: 
	pdflatex ReviewPaper
	bibtex ReviewPaper
	pdflatex ReviewPaper
	pdflatex ReviewPaper
#	open ReviewPaper.pdf


clean:
	rm ReviewPaper.dvi 
	rm ReviewPaper.aux 
	rm ReviewPaper.blg 
	rm ReviewPaper.log 
	rm ReviewPaper.out 


mktab: mktab.o  
	g++ $(COMP) mktab.o -lm -l$(F77LIB) \
	-o mktab

MkTab: MkTab.o
	g++ MkTab.o -o MkTab


.f.o:
	$(F77COMP) $(F_FLAGS) -c $< -o $*.o

.c.o:
	g++ $(C_FLAGS) -c $< -o $*.o





==> QCDfits_DIS_back.tex <==
% \subsection{QCD fits to DIS data}
\subsection{QCD fits to HERA data}

\label{sec:HERAPDF}

% The combination $ \sim 4 xU + xD$, where $xU = xu + xc$ ($xD = xd + xs + xb$) 
% denotes the pdf of
% up-like (down-like) quarks, is well constrained at low and medium Bjorken $x$
% via Neutral Current DIS; the scaling violations of $F_2$, i.e.
% its logarithmic dependence on the four-momentum transfer squared $Q^2$, give access
% to the gluon density at low and medium $x$; additional constraints from Charged
% Current DIS allow some separation between $U$ and $D$ to be made,
% although with a limited precision. As a result, QCD fits to HERA data alone
% give access to all parton distribution functions in the proton.


As seen in section~\ref{sec:expt}, the HERA experiments performed 
high precision measurements of NC and CC DIS in a large kinematic domain,
both in $e^+p$ and $e^-p$ collisions.
In particular:
\begin{itemize}
\item the precise measurement of the scaling violations of the structure function $F_2$ in NC DIS, i.e.
  its logarithmic dependence on the four-momentum transfer squared $Q^2$,
  gives access to the gluon density at low and medium $x$;
\item the precise measurement of $F_2$ in NC DIS at low and medium $x$
   sets strong constraints on the combination 
   $ 4 ( U + \bar{U} ) + ( D + \bar{D})$ where $U$ and $D$ denote the combined up-type and down-type 
   quark densities, $U = u + c$ and $D  =d + s + b$;
\item the CC DIS measurements provide two constraints:
   one on a linear combination of $D$ and $\bar{U}$ ($e^+ p$ data), and one on a 
   linear combination of $U$ and $\bar{D}$ ($e^- p$ data);
\item the measurement of $xF_3$ obtained from the difference of $e^+p$ and $e^-p$
  NC DIS cross sections provides a constraint on a linear combination of $U - \bar{U}$ 
  and $D - \bar{D}$.
\end{itemize}
As a result, good constraints can be obtained on the gluon density as well
as on $U$, $D$, $\bar{U}$ and $\bar{D}$ from HERA data alone.
The separation between $U$ and $D$, which is provided by the CC DIS measurements,
can be further improved, in global fits, by including e.g. DIS measurements
on a deuterium target which set a constraint on $ 4 ( D + \bar{D}) + ( U + \bar{U} )$.
In fits based only on inclusive DIS measurements,
separating further $U$, $D$, $\bar{U}$ and $\bar{D}$ along the individual
quark flavours mostly relies on assumptions.



\subsubsection{Fit of the combined HERA-I inclusive datasets}
\label{sec:HERAPDF1.0}

% The extraction of parton density functions performed using only the
% averaged H1 and ZEUS DIS measurements presented in section~\ref{sec:expt}
% is described in this paragraph. 
% This QCD analysis, leading to the HERAPDF1.0 pdfs, is described in more details in~\cite{:2009wt}.
The HERAPDF1.0 parton densities~\cite{:2009wt} were extracted using only the
averaged H1 and ZEUS DIS measurements presented in section~\ref{sec:expt}.
%
The averaged HERA dataset corresponds to $741$ cross section measurements: $528$ ($145$) measurements 
of $e^+ p$ ($e^- p$) NC DIS and  $34$ measurements of both $e^+ p$ and $e^- p$ CC DIS.
Following a cut $Q^2 > Q^2_{min}$ with $Q^2_{min} = 3.5$~GeV$^2$, imposed to remain in the kinematic domain where pQCD is
reliable, $592$ data points are included in the QCD fit of~\cite{:2009wt}.
%
% The QCD analysis is performed at the NLO within the $\overline{MS}$ renormalization
% scheme. The programme QCDNUM~\cite{QCDNUM} is used to evolve the PDFs according to the DGLAP
% equations and to calculate the light quark coefficient functions.
% The heavy quark coefficient functions are calculated within the
% general mass variable flavour number scheme of~\cite{hep-ph/9709442, hep-ph/0601245}.
The fit is performed at NLO within the
general mass variable flavour number scheme of~\cite{hep-ph/9709442, hep-ph/0601245}.
The starting scale is chosen to be slightly below the charm threshold,
$Q^2_0 = 1.9$~GeV$^2$.


The initial parton distributions\footnote{Since $c(x) =0$ and $b(x) = 0$ at the
chosen starting scale, $U(x) = u(x)$ and $D(x) = d(x) + s(x)$ at $Q^2_0$.}
$xf = xg, xu_v, x d_v, x \bar{U}$ and $x \bar{D}$
are parameterised at $Q^2_0$ using the generic form:
\begin{equation}
     xf(x) = A x^B (1-x)^C (1 + \epsilon \sqrt{x} + D x + E x^2)
 \label{eqn:generic_HERAPDF}
\end{equation}

% The normalisation parameters $A_{u_v}$ and $A_{d_v}$ are not free parameters
% in the fit, but are obtained from the other parameters via the number
% sum rules.
% Since the existing data have a limited sensitivity to the behaviour of
% the valence quark distributions at low $x$, it is assumed that
% $B_{u_v} = B_{d_v}$.
% Similarly, the behaviour of the up and down anti-quarks at low $x$ is assumed
% to be governed by the same power, $B_{\bar{U}} = B_{\bar{D}}$.
% The strange quark distribution, $x \bar{s} = f_s x \bar{D}$,  is expressed as 
% a $x-$independent fraction, $f_s = 0.31$, of the down-like sea at the starting scale.
% The normalisations of the $\bar{U}$ and $\bar{D}$ distributions
% are related by:
% \begin{eqnarray*}
%  A_{\bar{U}} = A_{\bar{D}} ( 1 - f_s )
% \end{eqnarray*}
% which, together with $B_{\bar{U}} = B_{\bar{D}}$, corresponds to the usual 
% assumption that $\bar{d} / \bar{u} \rightarrow 1$
% as $x \rightarrow 0$.
% Finally, the normalisation $A_g$ of the gluon distribution is derived from
% the momentum sum rule.
% These constraints reduce by $6$ the number of free parameters in the fit.

At low $x$ the assumptions $\bar{d} / \bar{u} \rightarrow 1$ as $x \rightarrow 0$
and $B_{u_v} = B_{d_v}$ are made, which together with the number and momentum sum rules,
removes $6$ free parameters of the fit.
The strange quark distribution, $x \bar{s} = f_s x \bar{D}$,  is expressed as
a $x-$independent fraction, $f_s = 0.31$, of the down-type sea at the starting scale.

A $9$-parameter fit is first performed by setting to zero all
$\epsilon$, $D$ and $E$ parameters in Eq.~\ref{eqn:generic_HERAPDF}.
These parameters are then introduced one by one, the best $10$-parameter
fit having $E_{u_v} \neq 0$. 
% As a result of this procedure, the central fit of HERAPDF1.0 is a
As a result\footnote{
Setting $E_{u_v} \neq 0$ and introducing an
eleventh parameter in the fit does not reduce the $\chi^2$ significantly,
with the exception of the fit having both $E_{u_v} \neq 0$ and $D_g \neq 0$.
However, the latter leads to very low valence quark distributions at high $x$,
with in particular $d_v (x) < \bar{d}(x)$. As this would dramatically fail to
describe e.g. $\nu p$ and $\nu d$ fixed target measurements of the structure
function $xF_3$~\cite{WA25}, this solution is discarded for the ``central fit".
However it is included in the parameterisation uncertainty discussed below.
},
the central fit of HERAPDF1.0 is a
$10$-parameter fit corresponding to the following parameterisation:
%
\begin{eqnarray}
xg(x) &=   & A_g x^{B_g} (1-x)^{C_g}  \label{eqn:herapdf_gluon}  \\
xu_v(x) &=  & A_{u_v} x^{B_{u_v}}  (1-x)^{C_{u_v}} \left[ 1 + E_{u_v} x^2 \right] ,  \label{eqn:herapdf_uv} \\
xd_v(x) &=  & A_{d_v} x^{B_{d_v}}  (1-x)^{C_{d_v}} ,  \label{eqn:herapdf_dv}  \\
x\bar{U}(x) &=  & A_{\bar{U}} x^{B_{\bar{U}}} (1-x)^{C_{\bar{U}}} ,  \label{eqn:herapdf_barU}   \\
x\bar{D}(x) &= & A_{\bar{D}} x^{B_{\bar{D}}} (1-x)^{C_{\bar{D}}} .   \label{eqn:herapdf_barD}
\end{eqnarray}



The fit has a $\chi^2$ of $574$ for $582$ degrees of freedom.
% As an example, the resulting PDFs at the starting scale $Q^2 = 1.9$~GeV$^2$ and at
% $Q^2 = 10$~GeV$^2$ are shown in Figure~\ref{Fig:hera_fits}.
% 
% %
% \begin{figure}[tb]
% \begin{tabular}{cc}
  % \includegraphics[width=0.5\columnwidth]{d09-158f18a.eps} &
  %  \includegraphics[width=0.5\columnwidth]{d09-158f18b.eps}  \\
  % \includegraphics[width=0.5\columnwidth]{d09-158f19a.eps} &
  % \includegraphics[width=0.5\columnwidth]{d09-158f19b.eps} 
 % \end{tabular}
% \caption{
% Distributions of valence quarks densities $x u_v$ and $x d_v$, of
% the gluon density $xg$ and of the density of sea quarks $xS$ obtained from
% the fit to the HERA-I dataset.
% }
% \label{Fig:hera_fits}
% \end{figure}
% %
Example PDFs at the scale $Q^2 = 10$~GeV$^2$ are shown in Fig.~\ref{Fig:hera_fits},
together with their uncertainties obtained as described below.

\begin{figure}[tbh]
% \centerline{\includegraphics[width=0.7\columnwidth]{d09-158f16.eps}} 
% \begin{tabular}{cc}
% \includegraphics[width=0.5\columnwidth]{d09-158f14.eps}  &
% \includegraphics[width=0.5\columnwidth]{d09-158f17.eps} 
% \end{tabular}
\begin{tabular}{cc}
\includegraphics[width=0.5\columnwidth]{d09-158f18b.eps} &
\includegraphics[width=0.5\columnwidth]{d09-158f19b.eps}
\end{tabular}
\caption{\sl
% Distributions of the combined up-type and down-type densities $U$, $D$, $\bar U$
% and $\bar D$, of the valence quarks densities $x u_v$ and $x d_v$, of
% the gluon density $xg$ and of the density of sea quarks $xS = 2x (\bar U + \bar D)$,
% and of the anti-quark densities $\bar u$, $\bar d$, $\bar s$ and $\bar c$ at
% $Q^2 = 10$~GeV$^2$, as obtained from the HERAPDF1.0 fit.
Distributions of valence quarks densities $x u_v$ and $x d_v$, of
the gluon density $xg$ and of the density of sea quarks $xS$ obtained from
the fit to the HERA-I dataset, at $Q^2 = 10$~GeV$^2$.
From~\cite{:2009wt}.
}
\label{Fig:hera_fits}
\end{figure}


The experimental uncertainty of the HERAPDF1.0 PDFs 
(shown as the red band in Fig.~\ref{Fig:hera_fits})
is determined using the Hessian method
described in section~\ref{sec:systematic_errors}, taking into account the $110$ sources of
systematic errors of the individual measurements together with their correlations.
The tolerance criterium $\Delta \chi^2 = 1$ is used to determine the $1 \sigma$ error bands.
Three additional errors (the largest), which correspond to the effect of treating differently
the systematic uncertainties in the averaging procedure of the H1 and ZEUS measurements,
are treated with the more conservative offset method\footnote{For the other $110$ sources
of systematic uncertainties, the offset method yields very similar results as the Hessian
method, since these uncertainties are smaller than the statistical uncertainties.}.
%
% As seen from Fig.~\ref{Fig:hera_fits}, 
Very good constraints are obtained on $U$,
$D$, $\bar{U}$ and $\bar{D}$, which are the combinations the measurements are
directly sensitive to, in a large range of $x$ extending down to $10^{-4}$ and up
to ${\cal{O}}(0.1)$. As expected, the best constraints are obtained on $U$, with an
uncertainty that remains below $10 \%$ for $x \lsim 0.5$.
The gluon PDF is also well constrained up to $x \sim 0.2$, and 
down to\footnote{Large uncertainties are actually obtained at low $x$ for the starting scale $Q^2 = 1.9$~GeV$^2$,
but are quickly
washed out by the DGLAP evolution.} $x \sim 10^{-4}$.


The model uncertainty, shown as the yellow band in Fig.~\ref{Fig:hera_fits}, is obtained
by varying the input values of $f_s$, $m_c$, $m_b$ and $Q^2_{min}$ and repeating the fit.
The largest effect comes from the variation of $f_s$ and the heavy quark masses, which
affects considerably the strange and charm densities.

Following~\cite{Aaron:2009kv}, an assessment of the additional uncertainty that
is introduced by the parameterisation choice is made in this analysis. 
This is particularly relevant since the number of parameters in the central
parameterisation of this analysis (Eq.~\ref{eqn:herapdf_uv}-\ref{eqn:herapdf_barD})
is rather small ($10$).  
The variation of the starting scale $Q^2_0$ is included in this 
parameterisation uncertainty. Indeed, when the DGLAP equations are used to
perform a backward evolution of the gluon distribution obtained from the central fit,
from $Q^2_0 = 1.9$~GeV$^2$
down to $1.5$~GeV$^2$, the resulting function cannot be fitted by the simple form
of Eq.~\ref{eqn:herapdf_gluon}. Consequently, repeating the fit with a lower starting scale
$Q^2_0 = 1.5$~GeV$^2$ results in large differences compared to the central fit if the same
parameterisation is kept, because Eq.~\ref{eqn:herapdf_gluon} is
not flexible enough to describe the gluon distribution at low scales.
Hence, when the fit is repeated with $Q^2_0 = 1.5$~GeV$^2$, additional freedom is
given for the gluon distribution by subtracting a term $A'_{g} x^{B'_g} (1-x)^{C'_g}$
to Eq.~\ref{eqn:herapdf_gluon}, as first suggested in~\cite{MSTW08}, where $C'_g$ is fixed
to a large value which ensures that this additional term does not contribute at high $x$.
Moreover, an additional fit is performed using the parameterisation of the central fit
but relaxing 
the assumption $B_{u_v} = B_{d_v}$.
Alternative
$11$-parameter fits with $E_{u_v} \neq 0$ are also considered, including those which lead
to good fit quality but peculiar behaviour at large $x$. 
An envelope is constructed, representing the maximal deviation, at each $x$ value,
between the central fit and the fits obtained using these parameterisation variations.
This envelope defines the parameterisation uncertainty of HERAPDF1.0
and is shown separately in Fig.~\ref{Fig:hera_fits} as the green band. 
The gluon and sea PDFs at low $x$ are mostly affected by the variation of $Q^2_0$
while at large $x$ (and over the whole $x$ range for the valence distributions), adding 
an eleventh parameter in the fit dominates the parameterisation
uncertainty. 
The total PDF uncertainty is obtained by adding in quadrature the experimental, model and
parameterisation uncertainties.
In particular, the parameterisation uncertainty increases considerably the uncertainty
of the gluon PDF at $x \sim 0.1$ and beyond.


% Syst error: DeltaChi2 = 1; use Hessian method for the 110 syst. sources
% of the measurements; use offset method for the ``procedural" errors,
% which correspond to a different treatment of systematic uncertainties
% in the averaging procedure.


\subsubsection{Improved flavour separation using fixed target DIS data}

As mentioned earlier, in fits using HERA data only, the flavour separation
is provided by the CC measurements.
In~\cite{ZEUS2003}, two fits were performed and compared:
\begin{itemize}
\item a fit which included ZEUS measurements of NC DIS at low $Q^2$, together with
 DIS data from fixed target experiments (in particular the 
NMC data on the ratio $F_2^d / F_2^p$, and the CCFR measurements on $xF_3$ which set
 strong constraints on the density of valence quarks);
\item a similar fit based on ZEUS data alone, where high $Q^2$ ZEUS data (on NC and CC DIS) were used instead
  of the fixed target data,  to provide information on the flavour separation.
\end{itemize}

This comparison showed that the gluon and
sea densities are mainly determined by the HERA data for $x$ below $\sim 0.1$.
However, the uncertainties of the valence distributions  were much smaller 
in the fit that included the fixed target data, in particular those of the
$d_{val}$ distribution.
Despite the much larger statistics at high $Q^2$ that has been collected by
the HERA experiments since~\cite{ZEUS2003}, the data from fixed target experiments
remain necessary for a precise determination of all quark densities\footnote{The preliminary fit HERAPDF1.5~\cite{MandyReview}, which uses the full
statistics collected by the H1 and ZEUS experiments, determines $d_{val}$   
to within $25\%$ up to $x \sim 0.25$. For larger $x$ values, $d_{val}$ is
poorly constrained by these data alone.}.




\subsubsection{Impact of jet data on the fits to HERA data}

As seen in Fig.\ref{Fig:hera_fits}, the precision on the gluon density
is limited at medium and high $x$ when only inclusive HERA data are used.
Adding HERA data from jet production in DIS and in photoproduction was
shown to lead to better constraints~\cite{ZEUS-JETS}.
%
Although HERA jet data do not bring strong constraints on the gluon density at high $x$
due to the limited statistics (better constraints at high $x$ are brought by Tevatron jet data),
they can be useful
for medium $x$, since HERA jet cross sections have small systematic uncertainties
(typically $5 \%$, a factor of at least $2$ smaller than the systematic uncertainties of 
jet cross sections measured by the Tevatron experiments, see section~\ref{exp:tevatron}).
% Fig.~\ref{fig:ZEUS_Jets} shows how the relative uncertainty on the gluon density improves
% when measurements of inclusive jet production at HERA (see Fig.~\ref{fig:Zeus_jets}) are
% also included in a fit based on HERA inclusive DIS data~\cite{ZEUS-JETS}.
%
For the fits performed using only HERA DIS inclusive data~\cite{ZEUS-JETS},
the uncertainty of the gluon density was reduced by
a factor of $\sim 2$ in the mid-$x$ region, $x = 0.01 - 0.4$, when measurements
of inclusive jet production at HERA (see Fig.~\ref{fig:Zeus_jets}) were included.
%
It is also interesting
to note that both fits, with and without the jet data, lead to the same shape for
the gluon density, indicating that there is no tension between the HERA jet and 
inclusive DIS data.
Similar conclusions were reached in preliminary fits using the full statistics
of HERA data~\cite{MandyReview}.


\subsubsection{Fits performed using preliminary combinations of HERA data}

Following HERAPDF1.0, several QCD fits have been performed to preliminary
combinations of HERA data. 
As for HERAPDF1.0, the extraction of the HERAPDF1.5 PDFs relies on inclusive DIS data only,
but a preliminary combination of H1 and ZEUS measurements from HERA-I and
HERA-II was used instead of the published HERA-I combined dataset.
This fit was also performed with additional freedom given to the gluon and the
$u_v$ parameterisation in Eq.~\ref{eqn:herapdf_gluon} and~\ref{eqn:herapdf_uv},
leading to $14$ free parameters instead of $10$ (HERAPDF1.5f). This extended parameterisation
was also used for the extraction of NNLO PDFs, HERAPDF1.5 NNLO. These fits, although unpublished, are available in the LHAPDF interface.
H1 and ZEUS jet data were added in order to extract the HERAPDF1.6 (NLO) PDFs.
The most recent preliminary fit, HERAPDF1.7, includes as well the $F_2^{c \bar{c}}$ measurements
and the data taken in $2007$ with a lower proton beam energy.
Further details can be found in~\cite{MandyReview, HERAWebPage}.

%
% %% \begin{figure}[tb]
% \centerline{
%   % \begin{tabular}{cc}
%   % \includegraphics[width=0.5\columnwidth]{DESY-05-050_4.ps} &
%   \includegraphics[width=0.5\columnwidth]{DESY-05-050_8.ps}
%   % \end{tabular}
% }
% \caption{
% % (left) Differential cross sections of inclusive jet production in DIS.
% % (right) 
% The relative uncertainty of the gluon density as a function of $x$ for
% several values of $Q^2$, when these jet data are included (light, yellow band)
% or are not included (dark, red band) in a QCD fit to ZEUS inclusive DIS data. From~\cite{ZEUS-JETS}.
% }
% \label{fig:ZEUS_Jets}
% \end{figure}
%

